Tensor network variational optimizations for real-time dynamics: application to the time-evolution of spin liquids

Within the Projected Entangled Pair State (PEPS) tensor network formalism, a simple update (SU) method has been used to investigate the time evolution of a two-dimensional U(1) critical spin-1/2 spin liquid under Hamiltonian quench [Phys. Rev. B 106, 195132 (2022)]. Here we introduce two different variational frameworks to describe the time dynamics of SU(2)-symmetric translationally-invariant PEPS, aiming to improve the accuracy. In one approach, after using a Trotter-Suzuki decomposition of the time evolution operator in term of two-site elementary gates, one considers a single bond embedded in an environment approximated by a Corner Transfer Matrix Renormalization Group (CTMRG). A variational update of the two tensors on the bond is performed under the application of the elementary gate and then, after symmetrization of the site tensors, the environment is updated. In the second approach, a cluster optimization is performed on a finite (periodic) cluster, maximizing the overlap of the exact time-evolved state with a symmetric finite-size PEPS ansatz. Observables are then computed on the infinite lattice contracting the infinite-PEPS (iPEPS) by CTMRG. We show that the variational schemes outperform the SU method and remain accurate over a significant time interval before hitting the entanglement barrier. Studying the spectrum of the transfer matrix, we find that the asymptotic correlations are very well preserved under time evolution, including the critical nature of the singlet correlations, as expected from the Lieb-Robinson (LR) bound theorem. Consistently, the system (asymptotic) boundary is found to bedescribed by the same Conformal Field Theory of central charge c = 1 during time evolution. We also compute the time-evolution of the short distance spin-spin correlations and estimate the LR velocity.

==> preamble.tex <==
\usepackage{graphicx}
\usepackage{graphics}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{amsfonts}
\usepackage{dsfont}
\usepackage{braket}
\usepackage{color}
\usepackage{braket,slashed}
\usepackage[mathscr]{euscript}
\definecolor{darkblue}{rgb}{0, 0, 0.8}
\usepackage[colorlinks=true, breaklinks=true, linkcolor=red, citecolor=blue, urlcolor=blue]{hyperref} 
%\usepackage{hyperref}
\usepackage{subfigure}
\usepackage{xfrac}
\usepackage{bm}
\usepackage{kantlipsum}
\usepackage{enumitem}
\usepackage{tikz}
\usepackage{framed}
\usepackage{graphicx}
\usepackage{subfigure}
%\usepackage{times}
\usepackage{cleveref}
\usepackage{adjustbox}


\usepackage{xcolor}

%\usepackage{geometry}
%\geometry{a4paper}
%\geometry{hmargin=2cm,vmargin=3cm}

\allowdisplaybreaks[1]

% code fonts
\newcommand{\code}[1]{\texttt{#1}}
\newcommand{\codestring}[1]{\code{\textquotesingle{}{#1}\textquotesingle{}}}
\newenvironment{partcode}{\begin{quote}\ttfamily}{\end{quote}}

\newenvironment{codeF}[1]{\begin{framed} \begin{quote} \par\code{#1} \vspace{\baselineskip} \par} {\end{quote} \end{framed}}

\newcommand{\functiond}[2]{ \begin{framed} \begin{quote} \par\code{#1} \vspace{\baselineskip} \par #2\end{quote} \end{framed}}

%\newenvironment{allintypewriter}{\ttfamily}{\par}

% symmetroes
\newcommand{\threej}[6]{\ensuremath{\begin{pmatrix} #1 & #2 & #3 \\ #4 & #5 & #6 \end{pmatrix}}}


% Special math fonts and notations
\newcommand{\T}{\ensuremath{\mathcal{T}}}
\newcommand{\h}[1]{\ensuremath{\hat{#1}}}
\renewcommand{\t}[1]{\ensuremath{\tilde{#1}}}
\newcommand{\ZZ}{\ensuremath{\mathbb{Z}}}
\newcommand{\CC}{\ensuremath{\mathbb{C}}}
\newcommand{\voperator}[1]{\ensuremath{\breve{#1}}}
\newcommand{\manifold}[1]{\ensuremath{\mathcal{#1}}}
\newcommand{\group}[1]{\ensuremath{\mathsf{#1}}}
\newcommand{\vectorspace}[1]{\ensuremath{\mathbb{#1}}}
\newcommand{\algebra}[1]{\ensuremath{\mathfrak{#1}}}
\newcommand{\bM}{\ensuremath{{\bar{M}}}}

% Math operators
\DeclareMathOperator*{\varmin}{min}
\DeclareMathOperator*{\varmax}{max}
\DeclareMathOperator*{\argmin}{arg\ min}
\DeclareMathOperator*{\argmax}{arg\ max}
\DeclareMathOperator{\order}{\mathscr{O}}
\DeclareMathOperator{\tr}{tr}
\DeclareMathOperator{\sign}{sgn}
\DeclareMathOperator{\End}{\mathbb{L}}
\DeclareMathOperator{\spanop}{span}
\DeclareMathOperator{\arctanh}{arctanh}
\DeclareMathOperator{\arccosh}{arccosh}
\DeclareMathOperator{\arcsinh}{arcsinh}

\newcommand{\commutator}[2]{\ensuremath{\left[#1,#2\right]}}
\newcommand{\anticommutator}[2]{\ensuremath{\left\{#1,#2\right\}}}
\newcommand{\sgn}{\ensuremath{\text{sgn}}}
\newcommand{\Pv}{\ensuremath{\text{Pv}\,}}



\newcommand{\one}{\mathds{1}}
\newcommand{\zero}{\mathds{0}}
\renewcommand{\dag}{^\dagger}
\newcommand{\pdag}{^{\phantom{\dagger}}}
\newcommand{\up}{{\uparrow}}
\renewcommand{\do}{\downarrow}
\newcommand{\updo}{{\uparrow\downarrow}}
\renewcommand{\d}{\ensuremath{\mathrm{d}}}
\newcommand{\e}{\ensuremath{\mathrm{e}}}
\newcommand{\grad}{\ensuremath{\vec{\nabla}}}
\newcommand{\ham}{\ensuremath{\hat{H}}}
\newcommand{\ovr}{\ensuremath{\overline{\bm{r}}}}
\newcommand{\orr}{\ensuremath{\overline{r}}}
\newcommand{\ic}{\ensuremath{i}}

\newcommand{\SU}{\ensuremath{\mathrm{SU}}}
\newcommand{\He}{\ensuremath{H_{\mathrm{ent}}}}
\newcommand{\vS}{\ensuremath{\vec{S}}}
\newcommand{\Z}{\ensuremath{\mathbb{Z}}}
\newcommand{\U}{\ensuremath{\mathrm{U}}}

\newcommand{\rket}[1]{\ensuremath{|#1)}}
\newcommand{\rbra}[1]{\ensuremath{(#1|}}
\newcommand{\rbraket}[1]{\ensuremath{(#1)}}
\newcommand{\Rket}[1]{\ensuremath{\left|#1\right)}}
\newcommand{\Rbra}[1]{\ensuremath{\left(#1\right|}}
\newcommand{\Rbraket}[1]{\ensuremath{\left(#1\right)}}

\newcommand{\vect}[1]{\ensuremath{\boldsymbol{#1}}}
\newcommand{\spst}{\ensuremath{\ket{\{s\}}}}
\newcommand{\E}[2]{\ensuremath{E^{#1}_{#2}}}
\renewcommand{\O}[2]{\ensuremath{O^{#1}_{#2}}}
\renewcommand{\H}[4]{\ensuremath{H^{#1#2}_{#3#4}}}
\newcommand{\I}[6]{\ensuremath{I^{#1#2#3}_{#4#5#6}}}
\newcommand{\HH}[6]{\ensuremath{H^{#1#2#3}_{#4#5#6}}}
\newcommand{\J}[4]{\ensuremath{J^{#1#2}_{#3#4}}}
\newcommand{\tA}{\ensuremath{A}}
\newcommand{\alphap}{\ensuremath{{\alpha'}}}
\newcommand{\betap}{\ensuremath{{\beta'}}}
\newcommand{\gammap}{\ensuremath{{\gamma'}}}
\newcommand{\perm}{\ensuremath{{\mathcal{P}}}}
\newcommand{\vv}{\ensuremath{\vect{v}}}
\newcommand{\Tr}{\ensuremath{\text{Tr}}}

\newcommand{\diagram}[1]{\;\vcenter{\hbox{\includegraphics[scale=0.32,page=#1]{./Figures/diagrams.pdf}}}\;}
\newcommand{\tmdiags}[2]{\;\vcenter{\hbox{\includegraphics[scale=#2,page=#1]{./Figures/tmdiags.pdf}}}\;}

\newcommand{\pepo}[1]{\;\vcenter{\hbox{\includegraphics{#1}}}\;}
\newcommand{\pepob}[2]{\;\vcenter{\hbox{\includegraphics[scale=#2]{#1}}}\;}

\newcommand{\lv}[1]{{\color{blue} #1}}
